BetaZero: Belief-State Planning for Long-Horizon POMDPs using Learned Approximations

Real-world planning problems, including autonomous driving and sustainable energy applications like carbon storage and resource exploration, have recently been modeled as partially observable Markov decision processes (POMDPs) and solved using approximate methods. To solve high-dimensional POMDPs in practice, state-of-the-art methods use online planning with problem-specific heuristics to reduce planning horizons and make the problems tractable. Algorithms that learn approximations to replace heuristics have recently found success in large-scale fully observable domains. The key insight is the combination of online Monte Carlo tree search with offline neural network approximations of the optimal policy and value function. In this work, we bring this insight to partially observable domains and propose BetaZero, a belief-state planning algorithm for high-dimensional POMDPs. BetaZero learns offline approximations that replace heuristics to enable online decision making in long-horizon problems. We address several challenges inherent in large-scale partially observable domains; namely challenges of transitioning in stochastic environments, prioritizing action branching with a limited search budget, and representing beliefs as input to the network. To formalize the use of all limited search information, we train against a novel $Q$-weighted visit counts policy. We test BetaZero on various well-established POMDP benchmarks found in the literature and a real-world problem of critical mineral exploration. Experiments show that BetaZero outperforms state-of-the-art POMDP solvers on a variety of tasks.

==> figures/ablations/ablation-figures.tex <==
\begin{figure*}[b!]
    \centering
    \begin{minipage}{0.69\textwidth}
        \resizebox{\textwidth}{!}{
            \includegraphics{figures/ablations/plot_ablation_q_weighting.pdf}
            \includegraphics{figures/ablations/plot_ablation_belief_rep.pdf}
            \includegraphics{figures/ablations/plot_ablation_action_selection.pdf}
    }
    \end{minipage}%%%
    \hspace*{3mm} % \hfill
    \begin{minipage}{0.3\textwidth}
        \resizebox{\textwidth}{!}{%
            \includegraphics{figures/results/z_sweep.pdf}
        }
    \end{minipage}

    \begin{minipage}[t]{0.69\textwidth}
        \caption{
        Ablation study in \textsc{LightDark}$(10)$.
        (Left) Learning is faster when policy network is trained using $Q$-weighted visit counts.
        (Middle) Incorporating belief uncertainty is crucial for learning.
        (Right) Action widening from the policy network shows significant improvement.
        The same red curves are shown and one std is shaded from three seeds with exponential smoothing with weight $0.6$.}
        \label{fig:ablations}
    \end{minipage}%%%
    \hspace*{3mm} % \hfill
    \begin{minipage}[t]{0.3\textwidth}
        \caption{Ablation study in \textsc{RockSample}$(20,20)$.
        Combining value and count information leads to the highest return. The diagonal is identical due to the $\argmax$ of \cref{eq:policy_q_weight}.}
        \label{fig:z_sweep}
    \end{minipage}
\end{figure*}

